Toward Multimodal Model-Agnostic Meta-Learning

Gradient-based meta-learners such as MAML are able to learn a meta-prior from similar tasks to adapt to novel tasks from the same distribution with few gradient updates. One important limitation of such frameworks is that they seek a common initialization shared across the entire task distribution, substantially limiting the diversity of the task distributions that they are able to learn from. In this paper, we augment MAML with the capability to identify tasks sampled from a multimodal task distribution and adapt quickly through gradient updates. Specifically, we propose a multimodal MAML algorithm that is able to modulate its meta-learned prior according to the identified task, allowing faster adaptation. We evaluate the proposed model on a diverse set of problems including regression, few-shot image classification, and reinforcement learning. The results demonstrate the effectiveness of our model in modulating the meta-learned prior in response to the characteristics of tasks sampled from a multimodal distribution.

==> text/intro-backup.tex <==
\section{Introduction}
\label{sec:intro}

%\sun{the first two sentences don't sound interesting at all.} Humans are naturally able to utilize experience from previous tasks for learning similar tasks with relatively little practice needed. Enabling machines to similarly utilize prior experience would be beneficial, because it would reduce the amount of training data needed and make training faster. One approach to achieving such fast adaptation in machine learning is to consider the problem of using prior information for rapidly learning new tasks a learning problem in its own right. These learning to learn approaches are collectively called meta-learning.
%\sun{we should mention multi-modal distribution in the first paragraph.}
%\sun{this first paragraph is ok if we are writing a book of meta-learning, but now we are writing a paper. the reviewers get bored easily. don't give them an impression that there is nothing new - this is just another random meta-learning paper}
%\sun{talk about how naturally this problem (learning a prior for multi-modal distributions) should have been address and why it's not how hard it is to machines).}

%Imagine that you watched a series of football tutorials from YouTube. There are several different skills you watched, and you would like to learn all of them. Despite the complexity and difference of the skills, humans like us can easily adapt to new skills based on our existing motor skills (\ie kicking). \jl{I am just outlining what it should be. Someone needs to (1) come up with a better example than football, and (2) improve sentences by making them more specific and connect sentences.}

% Getting exposed to a wide range of tasks can help us to learn a new skill quickly. Learning different skills does not make it slower to learn other skills. Learning basketball doesn't hurt learning baseball. 

%Imagine you are learning to swim. You know there are several different styles of swimming and you decide to learn a couple of them in order to maintain a good balance in the exercise. Mastering the different styles requires learning complex movements that are distinctive to the style in question. Luckily for you, humans can easily learn new motor skills based on the existing ones, which means you can learn backstroke faster after you've already learned the basics of breaststroke. More generally, it is natural for humans to learn sets of similar but different skills and expect faster learning the more skills you have from the set.

%Imagine you are learning to swim. You know there are several different styles of swimming and you decide to learn a couple of them in order to maintain a good balance in the exercise. Mastering the different styles requires learning complex movements that are distinctive to the style in question. Luckily for you, humans can easily adopt many motor skills, which have similar purpose and overlap to some degree, without the various skills interfering with each other. This means you can learn both backstroke and breaststroke without learning one making it hard to learn the other. More generally, it is natural for humans to learn sets of similar but different skills (\ie{skills coming from a multimodal distribution}) and they can even expect faster learning the more skills we have from the set.

% [theory 1] Humans are capable of effectively exploiting prior knowledge and experiences to acquire new skills as well as adapt to unseen/novel setup/environments(?).

% \Skip{
% %%% [example 1] 
% Humans are capable of effectively utilizing prior knowledge to acquire new skills as well as adapt to new environments.
% For example, imagine that we are learning how to carve on a snowboard on a mountain that we just arrived at.
% While we only know the basics of snowboarding and barely know the terrain, 
% we can still accomplish this feat quickly.
% %  because -- just like other humans, 
% % you are able to effectively utilize prior knowledge to acquire new skills and adapt to new environments.
% Even when the skill that we are interested in learning is only vaguely related to
% the set of skills that we have acquired in the past,
% we are usually able to exploit the relationship among skills and generalize.
% % This ability of generalizing to a wide range of vaguely related tasks 
% % ultimately allows us to efficiently master diverse skills recalling past related experiences.
% % In the same vein, 
% For the snowboarding example, our knowledge about skiing and skateboarding can play the role that prepares us for learning snowboarding skills more efficiently.
% }
% Similarly, can machines rapidly master a novel skill 
% based on a variety of related skills they have already acquired?

Recent advances in meta-learning offer machines a way to learn from
a distribution of tasks and adapt to a new task from the same
distribution using few samples.
% One (two) sentence survey of meta-learning
% Different approaches for engaging the task distribution exist.
% Optimization-based meta-learners~\citep{schmidhuber:1987:srl, bengio1992optimization, andrychowicz_learning_2016} learn updating functions or rules to optimize learner models.
Model-based meta-learning approaches~\citep{duan2016rl, wang2016learning, munkhdalai_meta_2017, mishra_simple_2017} 
propose to 
% design sophisticated architectures that are able to 
recognize the task identity from a few sample data and make 
the appropriate predictions by adjusting a model's state (\eg RNN's internal states).
Those methods demonstrate improved performance at the expense of engineering hand-designed architectures, yet the optimal strategy of designing a meta-learner for an arbitrary range of tasks may not be obvious to humans.
%{\color{red}[do their jobs]},
% a recurrent model is learned,
% learn an update rule and 
On the other hand, gradient-based meta-learning frameworks~\citep{finn_model-agnostic_2017, finn_probabilistic_2018, kim_bayesian_2018, lee_gradient-based_2018, grant_recasting_2018}
% dubbed \textit{gradient-based meta-learning},
seek an initialization of model parameters 
such that a small number of gradient updates will lead to fast learning on a new task,
offering the flexibility in the choice of models.
% and adapt rapidly by performing gradient descent steps.
% learns an initialization for gradient based adaptation, 
% FACT1: GBML is good
% Using gradient descent to adapt to a new task starting from a learned initialization
% Gradient-based meta-learning 
% These methods are able to generalize consistently
% to tasks that are extrapolations of those sampled from the task distribution
% by incorporating the positive inductive bias of gradient-based learning
% \citep{finn_meta-learning_2017}.
% FACT2: GBML cannot handle multimodal distributions

\Skip{
Optimization-based meta-learning approaches learn to optimize a learner model by optimizing learned parameters~\cite{schmidhuber:1987:srl, bengio1992optimization}, 
representing a learning as a reinforcement learning policy~\cite{li_learning_2016},
or learning update rules~\cite{andrychowicz_learning_2016, ravi_optimization_2016}.
Metric-based meta learners strive to learn a metric which can be used to compare two different samples effectively and perform tasks in the learned metric space~\cite{koch2015siamese, vinyals2016matching, snell_prototypical_2017, shyam2017attentive, Sung_2018_CVPR}.
Model-based meta-learning frameworks learn to recognize the identities of tasks and adjust the model state (\eg the internal state of an RNN) to fit the task~\cite{santoro_meta-learning_2016, duan2016rl, munkhdalai_meta_2017}.
While achieving impressive results on a wide range of tasks, those methods are not able to continually improve the performance during the meta-testing phase.
\cite{finn_model-agnostic_2017} and its extensions ~\cite{finn_probabilistic_2018, kim_bayesian_2018, lee_gradient-based_2018, grant_recasting_2018}, known as gradient-based meta-learning, aim to estimate a parameter initialization that provides a favorable inductive bias for fast adaptation.
However, assuming tasks are sampled from a concentrated distribution and pursuing a common initialization to all tasks can substantially limit the performance of such methods on multimodal task distributions where the center in the task space becomes ambiguous.
}

While most of the existing gradient-based meta-learners rely on a single initialization,
different modes of a task distribution can require substantially different parameters,
making finding an initialization that is a short distance away from all of them
infeasible.
% the drawback of relying on a single initialization is that the different modes
% of a task distribution can require substantially different parameters,
% making finding an initialization that is a short distance away from all of them infeasible.
When the modes of a task distribution are disjoint, we might be able to obtain a set of separate
meta-learners to master each mode.
However, this not only 
requires additional identity information about the modes, 
which is not always available or is ambiguous when the modes are not clearly disjoint,
but also eliminates the possibility of associating transferable knowledge across different modes of a task distribution.
% In order to do so, we do not want to merely associate separate models with each of the
% modes as that would make sharing information across the modes impossible.
To overcome this issue,
we aim to develop a meta-learner that is able to 
acquire a meta-learned prior and adapt quickly 
given tasks sampled from a multimodal task distribution.
% {\color{red}[talk about Probabilistic MAML, Bayesian MAML, etc. and why they don't address this issue well. (essentially they are still unimodal]}

% Meta-learners that are limited to using prior information from unimodal distributions
% fall short of the goal of fast adaptation, as multiple learners are required for fitting the task distribution.
% %
% \Skip{
% \risto{insert segue}
% Developing methods for gradient based meta-learning in multimodal task distribution
% would enable us to take advantage of the good generalization properties of gradient based meta-learning.
% %
% However, gradient based meta-learning in multimodal task distributions is challenging, as
% the learned initialization will have to work with tasks coming from all of the modes.
% While a lot of the information between the modes is shared -- otherwise it would not
% make sense to do meta-learning in the first place -- different modes still require
% specialization, which is hard to accommodate using the single initialization vector.
% }

%\risto{One published paper, I know off, talks about multimodal task distributions:
%\cite{finn_probabilistic_2018}, they say it's challenging for uncertainty estimation but don't
%explicitly say that GBML should struggle with it.}

% \sun{4th paragraph: our methods}
% \hx{I have wrote something, we can further improve this.}

% Instead, we leverage the task identification capabilities of model-based meta-learners to condition a gradient-based meta-learner on the task identity thus preconditioning the model for fast adaptation in that mode.

To this end, we leverage the strengths of the two main lines of existing meta-learning techniques: model-based and gradient-based meta-learning.
Specifically, we propose to augment gradient based meta-learners with 
the capability of generalizing across a multimodal task distribution. 
Instead of learning a single initialization point in the parameter space, 
we propose to first estimate the mode of a sampled task by examining task related samples.
Given the estimated task mode, our model then performs a step of \textit{model-based adaptation}
to modulate the meta-learned prior in the parameter space to fit the sampled task.
Then, from this model-based adapted meta-prior, a few steps of \textit{gradient-based adaptation}  are performed towards the target task
to progressively improve the performance on the task.
This main idea is illustrated in \myfig{fig:model}. 


% \Skip{
% The main contributions of this paper include a meta-learner that is able to 
% acquire a meta-learned prior and adapt quickly given tasks sampled from a multimodal task distribution
% by taking advantage of both model-based and gradient-based meta-learning.
% We evaluate the effectiveness of our proposed model on 
% a diverse set of different learning problems, including classification, regression, and reinforcement learning.
% We demonstrate that our model offers a better generalization ability compared to state-of-the-art meta-learners especially when task distributions are multimodal.
% }

%For both humans and machines, the easiest case for learning a new task is when the previous experience includes minor variations of the task. On one hand, humans are able to master multiple only vaguely related tasks and we benefit from having experience in those tasks when learning a new one.

%As a step towards enabling artificial agents to use information from a diverse distribution of previous experiences, we investigate the special \sun{don't make it sound special. it's natural to address this problem, and it is not just an increment from the current meta-learning paradigm.} case where the tasks come from a task distribution with multiple distinct modes.

%\sun{instead of saying existing meta-learners are useful, but we want to improve them, we should strongly say that meta-learning is not practical yet, and we are proposing the right meta-learner.}

%A new model, which combines ideas from both model based and gradient based meta-learning is central to our proposed approach. The model conditions a gradient based meta-learner on task embeddings computed by a model inspired by model based meta-learning. For finetuning the model to the new task, we follow the work in gradient-based meta-learning by \cite{finn_model-agnostic_2017}, where an initialization is learned such that good local optima for the tasks sampled from some task distribution are short distance away in the parameter space. We identify the sharing of the single initialization across the different modes making gradient based adaptation hard for multimodal task distributions and propose to use task embeddings to conditionally select submodels of the meta-learner for adaptation to the tasks from different modes.

\Skip{
\begin{figure*}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[height=130pt]{figures/mumomaml_teaser_2.pdf} &
    \includegraphics[height=130pt]{figures/mumomaml_model.pdf} \\
    (a) & (b)\\
    \end{tabular}
    
    \caption{
    (a) Diagram of multimodal model-agnostic meta-learning (\OurMethod) algorithm, which aims to acquire a meta-learned prior parameterized by $\theta$ and $\omega$, enabling fast adaptation to a task sampled from a multimodal distribution.
    Areas of different color indicate modes of tasks.
    (b) Overview of our model. Our model consists of two components: a model-based and gradient-based meta-learner. The former strives to identify the mode of a task distribution from a few samples and modulate the prior accordingly; the latter performs gradient updates to effectively yield better performance.
        \label{fig:illustration}
    }
\end{figure*}
}


==> text/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Optimization-based meta-learning approaches learn to optimize a learner model by 
optimizing learned parameters~\cite{schmidhuber:1987:srl, bengio1992optimization}, 
representing a learning as a reinforcement learning policy~\cite{li_learning_2016},
or learning update rules~\cite{andrychowicz_learning_2016, ravi_optimization_2016}.
Metric-based meta learners strive to learn a metric which can be used to compare two different samples effectively and perform tasks in the learned metric space~\cite{koch2015siamese, vinyals2016matching, snell_prototypical_2017, shyam2017attentive, Sung_2018_CVPR}.
Model-based meta-learning frameworks learn to recognize the identities of tasks and adjust the model state (\eg the internal state of an RNN) to fit the task~\cite{santoro_meta-learning_2016, duan2016rl, munkhdalai_meta_2017}.
While achieving impressive results on a wide range of tasks, those methods are not able to continually improve the performance during the meta-testing phase.
\cite{finn_model-agnostic_2017} and its extensions ~\cite{finn_probabilistic_2018, kim_bayesian_2018, lee_gradient-based_2018, grant_recasting_2018}, known as gradient-based meta-learning, aim to estimate a parameter initialization that provides a favorable inductive bias for fast adaptation.
However, assuming tasks are sampled from a concentrated distribution and pursuing a common initialization to all tasks can substantially limit the performance of such methods on multimodal task distributions where the center in the task space becomes ambiguous.
% In this work, we propose to exploit the strengths of both model-based and gradient-based meta-learners. Specifically, we utilize model-based learners' ability of identifying the mode of a task distribution to modulate meta-learned prior parameters to fit the model better to the mode. Then our model seek to rapidly improve the performance on the task afterwards by taking a few gradient steps.

\Skip{
As things stand right now, we are proposing a new kind of model for gradient-based meta-learning that uses the full training set as an additional input to condition the model on the task. For training the proposed model we use MAML \cite{finn_model-agnostic_2017}

\risto{a nice reference for this section is the table in \cite{metz_learning_2018}. Refer the reader there for a more comprehensive overview}

Our proposed is similar to the sequential meta-learning algorithms \cite{mishra_simple_2017,santoro_meta-learning_2016} in that we use a sequence model to process the training set and train that sequence model on the combined loss over multiple tasks. The difference to the sequential meta-learning models is that in our model, we rely on gradient-based meta-learning for the adaptation instead of learning the meta-learning algorithm within the recurrent model. \risto{write about the favorable performance of GMBL over MBML and refer to meta-learning and univ \cite{finn_meta-learning_2017} + tristan deleu \cite{deleu_reproducibility_2018} + \cite{rusu_meta-learning_2018}}

\risto{GBML papers like reptile \cite{nichol_first-order_2018}. Comment on MT-Nets using masking + learned linear layers to improve over maml \cite{lee_gradient-based_2018}. one-shot visual imit. learning for maml extensions \cite{finn_one-shot_2017}.} Our proposed model is also similar to the model proposed in \cite{rusu_meta-learning_2018}, which generates task specific model parameters using a VAE-like model and optimizes the latent embedding using MAML. \risto{LEO generates parameters conditional on the training set, but the decrease in performance compared to a random prior is small. The author's argue that the important part is doing MAML in the smaller latent embedding space compared to the full parameter space. Should we consider limiting MAML update step only to parts of our model?} \risto{LEO looks it's uploaded on arxiv using the ICLR template. Dunno if that matters.} Another gradient-based meta-learning approach is presented in \cite{ravi_optimization_2016} where an optimizer is learned to quickly adapt the model to the current task.

\risto{probabilistic MAML papers for also tackling something like multimodal task distributions \cite{finn_probabilistic_2018}, \cite{kim_bayesian_2018}, \cite{grant_recasting_2018}. Is there a citation for Grant's ICML 2018 poster?}

\risto{other meta-learning algorithms. cite Munkhdalai \cite{munkhdalai_meta_2017} cuz he's nice, modular meta-learning \cite{alet_modular_2018} bears some distant similarity our model, }

\risto{various ways of conditioning. Sigmoid gates similar to \cite{serra_overcoming_2018}, Film \cite{perez_film:_2017}, TADAM seems related \cite{oreshkin_tadam:_2018}}
}

